Guionnet-Jones-Shlyakhtenko subfactors associated to finite-dimensional Kac algebras

We analyse the Guionnet-Jones-Shlyakhtenko construction for the planar algebra associated to a finite-dimensional Kac algebra and identify the factors that arise as finite interpolated free group factors.

==> README.tex <==

This is the second version posted to the arXiv. Spelling mistake
of Roland corrected only.
